Letter of Intent: The Precision IceCube Next Generation Upgrade (PINGU)

The Precision IceCube Next Generation Upgrade (PINGU) is a proposed low-energy in-fill array of the IceCube Neutrino Observatory. Leveraging technology proven with IceCube, PINGU will feature the world's largest effective volume for neutrinos at an energy threshold of a few GeV, improving the sensitivity to several aspects of neutrino oscillation physics at modest cost. With its unprecedented statistical sample of low-energy atmospheric neutrinos, PINGU will have highly competitive sensitivity to $\nu_{\mu}$ disappearance, the $\theta_{23}$ octant, and maximal mixing, will make the world's best $\nu_{\tau}$ appearance measurement, allowing a unique probe of the unitarity of the PMNS mixing matrix, and will be able to distinguish the neutrino mass ordering at $3\sigma$ significance with less than 4 years of data. PINGU can also extend the indirect search for solar WIMP dark matter complimentary to the on-going and planned direct dark matter experiments. At the lower end of the energy range, PINGU may use neutrino tomography to directly probe the composition of the Earth's core. With its increased module density, PINGU will improve IceCube's sensitivity to galactic supernova neutrino bursts and enable it to extract the neutrino energy spectral shape.

==> Acknowledgements.tex <==
We acknowledge the support from the following agencies: U.S. National Science Foundation-Office of Polar Programs, U.S. National Science Foundation-Physics Division, University of Wisconsin Alumni Research Foundation, the Grid Laboratory Of Wisconsin (GLOW) grid infrastructure at the University of Wisconsin - Madison, the Open Science Grid (OSG) grid infrastructure; U.S. Department of Energy, and National Energy Research Scientific Computing Center, the Louisiana Optical Network Initiative (LONI) grid computing resources; Natural Sciences and Engineering Research Council of Canada, WestGrid and Compute/Calcul Canada; Swedish Research Council, Swedish Polar Research Secretariat, Swedish National Infrastructure for Computing (SNIC), and Knut and Alice Wallenberg Foundation, Sweden; German Ministry for Education and Research (BMBF), Deutsche Forschungsgemeinschaft (DFG), Helmholtz Alliance for Astroparticle Physics (HAP), Initiative and Networking Fund of the Helmholtz Association, Germany; Fund for Scientific Research (FNRS-FWO), FWO Odysseus programme, Flanders Institute to encourage scientific and technological research in industry (IWT), Belgian Federal Science Policy Office (Belspo); Marsden Fund, New Zealand; Australian Research Council; Japan Society for Promotion of Science (JSPS); the Swiss National Science Foundation (SNSF), Switzerland; National Research Foundation of Korea (NRF); Villum Fonden, Danish National Research Foundation (DNRF), Denmark


==> FrontMatter-Hierarchy.tex <==
\begin{frontmatter}

\title{The Precision IceCube Next Generation Upgrade (PINGU)\\ (Version: \today)}

\input{AuthorList}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{abstract}

{\bf Include authors not on the standard IceCube list!}

(PINGU LoI abstract not yet written.)

\end{abstract}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{keyword}

% Max 6 keywords

neutrinos \sep
neutrino oscillations \sep
neutrino hierarchy \sep

\end{keyword}

\end{frontmatter}

